Clock Diffusion: Efficient Semi-Autoregressive Continuous Diffusion Language Models

Recent works on continuous diffusion for discrete data have demonstrated performance on par with comparable discrete diffusion models. However, these continuous counterparts lack key features that are essential to practical use as language models, namely variable-length generation and support for a key-value cache, and they still lag behind the frontier of autoregressive and discrete diffusion quality. In this work, we address these limitations. We do so by introducing a model parameterization that uses position-dependent noise schedules to define semi-autoregressive (SAR) continuous diffusion language models (DLMs). Together with efficient training and sampling algorithms, we call this framework Clock Diffusion, and we present two special cases of our method: block and sliding window generation. We then define ClockDLMs, a family of Gaussian DLMs based on sliding window Clock Diffusion that attain state-of-the-art diffusion likelihood bounds on OpenWebText, even beating the performant block SAR discrete diffusion models. ClockDLMs trained on TinyGSM also substantially outperform continuous baselines on the GSM8K benchmark and match and exceed comparable SAR discrete diffusion models. Finally, building on our parameterization, we propose more efficient samplers that we dub Cache Grab, which adapt techniques from accelerated inference in discrete diffusion, such as committing tokens whose probabilities exceed a confidence threshold and self-speculative decoding, further improving our models' quality and efficiency.

==> figures/cache_grab_compact.tex <==
% Cache Grab sampling, COMPACT (9 slots, window 4) for the graphical abstract.
% Generated from cache_grab.tex; keep the two in sync if the visual language changes.
%
% Required in the manuscript preamble:
%   \usepackage{tikz}
%   \usetikzlibrary{arrows.meta}
%
% Visual language is shared with figures/clock_diffusion.tex (the graphical
% abstract): green = committed to the KV cache, purple = active window, grey
% dashed = not started; a latent is zero-mean Gaussian speckle whose amplitude
% is that position's local clock, over a constant pale ground, with the target
% token overlaid; the dial above an active position is its local clock.
%
% Rows are consecutive denoiser calls. Levels run 0 (denoised) to \cgLmax
% (pure noise) and drop by one per row, so a position can be tracked down the
% figure. The pseudo-random stream is seeded from the SLOT only, never the row,
% so each position keeps its noise realisation as it is denoised.
%
% NOTE: lines outside the tikzpicture must end in %.
%
\begingroup%
\definecolor{cgCache}{HTML}{3F8A5C}%
\definecolor{cgWin}{HTML}{2362B3}%
\definecolor{cgGhost}{HTML}{667085}%
\definecolor{cgTray}{HTML}{E7EFEA}%
\definecolor{cgInk}{HTML}{25232A}%
%
\def\cgP{0.97}% slot pitch
\def\cgW{0.90}% cell width
\def\cgH{0.54}% cell height
\def\cgR{0.125}% local clock radius
\def\cgLmax{6}% level of a fresh token
\def\cgBR{1.02}% bracket height above a row
\def\cgwords{the,cat,sat,on,the,red,mat,and,lay,by,the,old,oak}%
%
% local clock dial: {slot}{y}{u}{colour}
\newcommand{\cgdial}[4]{%
 \pgfmathsetmacro{\cgx}{\cgP*(#1-1)+0.5*\cgW}%
 \pgfmathsetmacro{\cga}{90-(1-#3)*360}%
 \fill[#4!12] (\cgx,#2) circle (\cgR);%
 \ifdim #3pt<1pt%
   \fill[#4!85] (\cgx,#2) -- ++(90:\cgR)%
     arc[start angle=90, end angle=\cga, radius=\cgR] -- cycle;%
 \fi%
 \draw[#4,line width=0.35pt] (\cgx,#2) circle (\cgR);}%
%
% active position: speckle + emerging token + its clock. {slot}{ybot}{level}{word}
\newcommand{\cgtok}[4]{%
 \pgfmathsetmacro{\cgx}{\cgP*(#1-1)}%
 \pgfmathsetmacro{\cgu}{#3/\cgLmax}%
 \path[fill=cgWin!13] (\cgx,#2) rectangle ++(\cgW,\cgH);%
 \pgfmathsetseed{\numexpr 1013+617*#1\relax}%
 \pgfmathsetmacro{\cgsw}{\cgW/12}%
 \pgfmathsetmacro{\cgsh}{\cgH/8}%
 \begin{scope}%
 \clip (\cgx,#2) rectangle ++(\cgW,\cgH);%
 \foreach \ci in {0,...,11}{%
  \foreach \cj in {0,...,7}{%
   \pgfmathsetmacro{\cgg}{(rand+rand+rand)*0.62}%
   \pgfmathsetmacro{\cgo}{min(0.92,abs(\cgg)*\cgu)}%
   \pgfmathtruncatemacro{\cgup}{\cgg>0 ? 1 : 0}%
   \ifnum\cgup=1%
     \path[fill=cgWin!88!black,opacity=\cgo]%
       (\cgx+\cgsw*\ci,#2+\cgsh*\cj) rectangle ++(\cgsw,\cgsh);%
   \else%
     \path[fill=white,opacity=\cgo]%
       (\cgx+\cgsw*\ci,#2+\cgsh*\cj) rectangle ++(\cgsw,\cgsh);%
   \fi%
  }}%
 \end{scope}%
 \pgfmathsetmacro{\cgfo}{#3<2 ? 0 : 0.60}%
 \pgfmathsetmacro{\cgto}{1-0.12*#3}%
 \node[font=\small,text=cgInk,inner sep=0.7pt,rounded corners=0.5pt,%
       fill=white,fill opacity=\cgfo,text opacity=\cgto]%
   at (\cgx+0.5*\cgW,#2+0.5*\cgH) {#4};%
 \draw[cgWin!55,line width=0.35pt,rounded corners=0.8pt]%
   (\cgx,#2) rectangle ++(\cgW,\cgH);%
}%
%
% not-yet-started slot: {slot}{ybot}
\newcommand{\cgghost}[2]{\pgfmathsetmacro{\cgx}{\cgP*(#1-1)}%
 \draw[cgGhost!50,densely dashed,line width=0.4pt,rounded corners=0.8pt]%
   (\cgx,#2) rectangle ++(\cgW,\cgH);}%
%
% KV cache tray with committed words: {last cached slot}{ybot}
\newcommand{\cgtray}[2]{\pgfmathsetmacro{\cgfr}{\cgP*#1-0.10}%
 \path[fill=cgTray,rounded corners=2pt] (-0.07,#2) rectangle (\cgfr,#2+\cgH);%
 \foreach \cgwq [count=\cgi from 1] in \cgwords{\ifnum\cgi<\numexpr#1+1\relax%
   \pgfmathsetmacro{\cgxc}{\cgP*(\cgi-1)+0.5*\cgW}%
   \node[font=\small,text=cgInk,inner sep=0] at (\cgxc,#2+0.5*\cgH) {\cgwq};\fi}%
 \draw[cgCache,line width=1.4pt] (\cgfr,#2-0.03) -- (\cgfr,#2+\cgH+0.03);}%
%
% set bracket: {xa}{xb}{y}{style}
\newcommand{\cgspan}[4]{\draw[#4]%
 ({#1},{#3-0.07})--({#1},{#3})--({#2},{#3})--({#2},{#3-0.07});}%
%
% all three set brackets: {ybot}{cache}{win first}{win last}{ghost first}{ghost last}
\newcommand{\cgsets}[6]{%
 \pgfmathsetmacro{\cgy}{#1+\cgBR}%
 \cgspan{-0.07}{\cgP*#2-0.10}{\cgy}{cgCache,line width=1.4pt}%
 \cgspan{\cgP*(#3-1)}{\cgP*(#4-1)+\cgW}{\cgy}{cgWin,line width=1.4pt}%
 \ifnum#5>#6\else\cgspan{\cgP*(#5-1)}{\cgP*(#6-1)+\cgW}{\cgy}%
   {cgGhost,line width=0.9pt,densely dashed}\fi}%
%
% ready-to-grab outline: {first}{last}{ybot}
\newcommand{\cgready}[3]{\pgfmathsetmacro{\cga}{\cgP*(#1-1)-0.025}%
 \pgfmathsetmacro{\cgb}{\cgP*(#2-1)+\cgW+0.025}%
 \draw[cgCache,line width=1.1pt,rounded corners=1.5pt]%
   (\cga,#3-0.025) rectangle (\cgb,#3+\cgH+0.025);}%
%
% one arrow per token: {first}{last}{ytop}{ybot}{style}
\newcommand{\cgflow}[5]{\foreach \cgs in {#1,...,#2}{%
  \pgfmathsetmacro{\cgxc}{\cgP*(\cgs-1)+0.5*\cgW}%
  \draw[#5] (\cgxc,#3) -- (\cgxc,#4);}}%
%
\begin{tikzpicture}[x=1cm,y=1cm,
  grabarrow/.style={cgCache,line width=1.5pt,-{Stealth[length=4.5pt,width=4.5pt]}},
  admitarrow/.style={cgWin,line width=1.2pt,densely dashed,
                     -{Stealth[length=4.5pt,width=4.5pt]}}]

% ============ row n : cache 1-3 | window 4-9 | not started 10-13 ==========
\cgtray{2}{0}
\foreach \cgL/\cgwq [count=\cgj from 0] in {0/sat,1/on,3/the,5/red}{%
  \pgfmathtruncatemacro{\cgsl}{3+\cgj}\cgtok{\cgsl}{0}{\cgL}{\cgwq}}
\foreach \cgsl in {7,...,9}{\cgghost{\cgsl}{0}}
\cgsets{0}{2}{3}{6}{7}{9}
\cgready{3}{4}{0}
\node[font=\small,text=cgCache,anchor=base] at ({0.5*(\cgP*2-0.17)},{\cgBR+0.10})
  {KV cache};
\node[font=\small,text=cgWin,anchor=base] at ({0.5*(\cgP*7+\cgW)},{\cgBR+0.10})
  {active window};
\node[font=\small,text=cgGhost,anchor=base] at ({0.5*(\cgP*14+\cgW)},{\cgBR+0.10})
  {not started};

% ---- gutter n -> n+1 ----
\cgflow{3}{4}{-0.06}{-0.78}{grabarrow}
\node[font=\small,text=cgCache,anchor=north,fill=white,inner sep=1pt] at ({0.5*(\cgP*2+\cgP*3+\cgW)},-0.84)
  {\textbf{grab 2} $\to$ cache};
\cgflow{7}{8}{-0.06}{-0.78}{admitarrow}
\node[font=\small,text=cgWin,anchor=north,fill=white,inner sep=1pt] at ({0.5*(\cgP*6+\cgP*7+\cgW)},-0.84)
  {admit 2 $\mathbf{z}_1\!\sim\!\mathcal{N}(\mathbf{0},\mathbf{I})$};

% ============ row n+1 : cache 1-5 | window 6-11 | not started 12-13 =======
\cgtray{4}{-2.25}
\foreach \cgL/\cgwq [count=\cgj from 0] in {0/the,2/red,4/mat,6/and}{%
  \pgfmathtruncatemacro{\cgsl}{5+\cgj}\cgtok{\cgsl}{-2.25}{\cgL}{\cgwq}}
\cgghost{9}{-2.25}
\cgsets{-2.25}{4}{5}{8}{9}{9}
\cgready{5}{5}{-2.25}

% ---- gutter n+1 -> n+2 ----
\cgflow{5}{5}{-2.31}{-3.03}{grabarrow}
\node[font=\small,text=cgCache,anchor=north,fill=white,inner sep=1pt] at ({0.5*(\cgP*4+\cgP*4+\cgW)},-3.09)
  {\textbf{grab 1} $\to$ cache};
\cgflow{9}{9}{-2.31}{-3.03}{admitarrow}
\node[font=\small,text=cgWin,anchor=north,fill=white,inner sep=1pt] at ({0.5*(\cgP*8+\cgP*8+\cgW)-1.0},-3.09)
  {admit 1 $\mathbf{z}_1\!\sim\!\mathcal{N}(\mathbf{0},\mathbf{I})$};

% ============ row n+2 : cache 1-6 | window 7-12 | not started 13 ==========
\cgtray{5}{-4.50}
\foreach \cgL/\cgwq [count=\cgj from 0] in {0/red,1/mat,3/and,5/lay}{%
  \pgfmathtruncatemacro{\cgsl}{6+\cgj}\cgtok{\cgsl}{-4.50}{\cgL}{\cgwq}}

\cgsets{-4.50}{5}{6}{9}{10}{9}
\cgready{6}{6}{-4.50}

% ---- row labels ----
% \foreach \cgy/\cglab in {0.27/{$n$},-1.51/{$n{+}1$},-3.29/{$n{+}2$}}{%
%   \node[font=\small,text=cgGhost!85!black,anchor=east] at (-0.20,\cgy) {\cglab};}
% global time axis
\draw[cgGhost,line width=1.0pt,-{Stealth[length=4.5pt,width=4.5pt]}]
  (-0.45,\cgBR-0.25) -- (-0.45,-3.62);
\node[font=\small,text=cgGhost,rotate=90,anchor=south]
  at (-0.45,-1.70) {\textit{Global diffusion time} $\downarrow$};
\end{tikzpicture}%
\endgroup%

